Mining Behavioral Patterns from Millions of Android Users

The prevalence of smart mobile devices has promoted the popularity of mobile applications (a.k.a. apps). Supporting mobility has become a promising trend in software engineering research. This article presents an empirical study of behavioral service profiles collected from millions of users whose devices are deployed with Wandoujia, a leading Android app store service in China. The dataset of Wandoujia service profiles consists of two kinds of user behavioral data from using 0.28 million free Android apps, including (1) app management activities (i.e., downloading, updating, and uninstalling apps) from over 17 million unique users and (2) app network usage from over 6 million unique users. We explore multiple aspects of such behavioral data and present patterns of app usage. Based on the findings as well as derived knowledge, we also suggest some new open opportunities and challenges that can be explored by the research community, including app development, deployment, delivery, revenue, etc.

==> chaps/preference.tex <==
\subsection{Is User Rating Always Coherent with App Management Activities?}


%\subsection{Leveraging App Management Activity Sequence}
%Above we demonstrated that only the amount of management activities could not well align with the user preferences. Then, we want to leverage the sequences of management activities to make further analysis. 

 We are motivated to find all such sequential indicators and combine them in a systematic way. 

\subsubsection{A Prediction Analysis}
Motivated by the sequential indicators, we move on to build a machine learning algorithm that predicts the \emph{likerate} of apps, with many possible sequential patterns of user activities as features. To evaluate the predictor, we randomly hold out 10\% of apps as test set and use the rest 90\% for training. As described before, user ratings are trustful only when there are abundant of them. We therefore only use the apps with at least 5 ratings in the test set to evaluate the prediction algorithms, treating the likerate of these apps as the ground-truth. To be specific, we have 50,143 apps in training set and 5,572 in the test set. In the test set, 2,195 apps have at least 5 ratings and are used in evaluation.

Let us use $D$ to represent a downloading activity, $P$ for updating and $U$ for uninstallation. We construct a D/P/U sequence for each user-app pair. For example, the sequence ``DPPUD'' indicates that the user downloaded the app, updated it twice, uninstalled it and then decided to re-install it. We count the occurrences of unigrams and bigrams, namely D, P, U, DD, DP, DU, PD, PP, PU, UD, UP, UU in every activity sequence and aggregate the counts over all sequences for an app. This gives us 12 numerical features, including the number of sequences as the 13th feature. 

Notice that some bigram features like ``UP'' (uninstallation followed by updating) might sound confusing as in reality one cannot update an app without installing it first. This is because activities not conducted through the Wandoujia management app are not logged. Also, a sequence does not necessarily begin with an ``D,'' since the app may be preloaded or the user might install an app before the five-month period and thus it is not captured in our log.

We first label apps in the training set with $likerate \ge 0.5$ as positive and the rest as negative, and then use them to train an \textit{Support Vector Machine (SVM)}. We apply the trained classifier to the test set, and generate the estimated probability of each app being positive. We also perform an \textit{Support Vector Regression (SVR)} to estimate the likerate. Both models can give us a numerical prediction for each app instead of a binary prediction. We evaluate the predictions using three metrics: the \textit{mean average precision (MAP)}, an classic metric in information retrieval used to evaluate a ranked list of results~\cite{manning2008introduction}; \textit{Pearson's $r$} which reports the correlation between the predicted likerate and the ground truth; and \textit{Spearman's $\rho$} which reports the rank correlation between the predicted and true likerate. The results are summarized in Table \ref{tab:performance}. Both SVM and SVR are performed by using the LibSVM package (Version 3.20)~\cite{CC01a}.
%cite chris manning
%cite libsvm

\begin{table}[htbp]
\caption{Comparison of the predictive power of different models. SVM and SVR are comparable, while AAMA makes better predictions of the likerate. }
\label{tab:performance}
\centering
\begin{tabular}{|l|c|c|c|}
\hline
				& MAP 			& Pearson's $r$ 	& Spearman's $\rho$ \\
\hline
SVM  			& 0.7595 		& 0.0435			& 0.0609	\\
\hline
SVR				& 0.7576		& 0.0367			& 0.0548	\\
\hline
AAMA	*		& 0.8240		& 0.1955			& 0.2009	\\
\hline		
\end{tabular}
\small

* AAMA is the probabilistic model that will be presented in Section 5. The results are presented here for an easy comparison. 
\end{table}


